DavIR: Data Selection via Implicit Reward for Large Language Models

We introduce DavIR, a model-based data selection method for post-training Large Language Models. DavIR generalizes Reducible Holdout Loss to core-set selection problem of causal language modeling, and quantifies the learnability of a given datum with respect to a pre-trained LLM based on relative reduction in loss during fine-tuning, a metric we show to be closely related to the implicit reward model described in Direct Preference Optimization (DPO). We show that 6% of Alpaca dataset selected with DavIR can steer both the LLaMA and Gemma model family to produce superior performance compared to the same models trained on the full 52K dataset. We also show that Alpaca dataset compressed with DavIR can be combined with GSM8K dataset to effectively balance open-domain freeform QA and mathematical reasoning capabilities. Finally, we apply the DavIR objective to DPO and develop a normalized DavIR-DPO objective which improves alignment performance of Zephyr-7B-SFT model by 8% (relative) on AlpacaEval, compared against training on vanilla DPO objective.

==> main/abstract.tex <==
% Supervised Fine-tuning (SFT) is a pivotal step in aligning Large Language Models (LLMs) with specific task requirements. The choice of fine-tuning data significantly impacts the model's performance, traditionally based on data quality and distribution. However, we introduce a novel dimension in data selection: learnability. The process of SFT is considered a means of unlocking the capabilities of pretrained models. However, since different models possess varying abilities, the data suitable for each model may differ as well. We define data's suitability for effective learning by the model as its learnability. We propose the \textbf{Lo}ss \textbf{Ba}sed \textbf{S}FT Data \textbf{S}election (LoBaSS) method, which employs data learnability as a guiding criterion for safe, efficient, and high-quality data selection. In experiments with 7B and 13B models, our method outperforms full-data fine-tuning with just 6\% of the data. With 16.7\% of the data, LoBaSS achieves a balance in the model's capabilities for both conversation and mathematical domains. Our work extends the scope and paving the way for SFT data construction and selection by introducing the concept of learnability.


% \hynote{Supervised Fine-Tuning (SFT) serves as a crucial phase in aligning Large Language Models (LLMs) to specific task prerequisites. The selection of fine-tuning data profoundly influences the model’s performance, a choice traditionally grounded in data quality and distribution. However, this paper introduces an innovative dimension in data selection: learnability. SFT is regarded as a technique for unlocking the potential of pretrained models. However, given that different models have disparate capabilities, the data appropriate for one may not suit another. Thus, we introduce the term ``learnability" to define the suitability of data for effective learning by the model. We present the \textbf{Lo}ss \textbf{Ba}sed \textbf{S}FT Data \textbf{S}election (LoBaSS)  method, utilizing data learnability as the principal criterion for the selection of secure, efficient, and high-quality data. This method provides a nuanced approach, allowing the alignment of data selection with inherent model capabilities, ensuring optimal compatibility and learning efficiency. In experimental comparisons involving 7B and 13B models, our LoBaSS method surpasses the full-data fine-tuning, requiring merely 6\% of the data. When employing 16.7\% of the data, LoBaSS harmonizes the model’s capabilities across conversational and mathematical domains, proving its efficacy and adaptability. } 

Supervised Fine-Tuning (SFT) serves as a crucial phase in aligning Large Language Models (LLMs) to specific task prerequisites. The selection of fine-tuning data profoundly influences the model’s performance, whose principle is traditionally grounded in data quality and distribution. In this paper, we introduce a new dimension in SFT data selection: learnability. This new dimension is motivated by the intuition that SFT unlocks capabilities acquired by a LLM during the pretraining phase. Given that different pretrained models have disparate capabilities, the SFT data appropriate for one may not suit another. Thus, we introduce the term ``learnability" to define the suitability of data for effective learning by the model. We present the \textbf{Lo}ss \textbf{Ba}sed \textbf{S}FT Data \textbf{S}election (LoBaSS)  method, utilizing data learnability as the principal criterion for the selection SFT data. This method provides a nuanced approach, allowing the alignment of data selection with inherent model capabilities, ensuring optimal compatibility and learning efficiency. In experimental comparisons involving 7B and 13B models, our LoBaSS method is able to achieve comparable results with 800 data points (1.5\%) and surpass full-data fine-tuning at merely 6\% of the total training data. When employing 16.7\% of the data, LoBaSS harmonizes the model’s capabilities across conversational and mathematical domains, proving its efficacy and adaptability.

% \htzhou{Model Knows Best How to Align}

% \htzhou{Learnability-Driven Data Selection for LLM Fine-Tuning}

% \htzhou{Learnability Matters for Fine-Tuning Data}


